Multi-phase characterization of AGN winds in 5 local type-2 quasars

We present MEGARA (Multi-Espectr\'ografo en GTC de Alta Resoluci\'on para Astronom\'ia) Integral Field Unit (IFU) observations of 5 local type-2 quasars (QSO2s, z $\sim 0.1$) from the Quasar Feedback (QSOFEED) sample. These active galactic nuclei (AGN) have bolometric luminosities of 10$^{45.5-46}$ erg/s and stellar masses of $\sim$10$^{11}$ M$_{\odot}$. We explore the kinematics of the ionized gas through the [O~III]$\lambda$5007 $\r{A}$ emission line. The nuclear spectra of the 5 QSO2s, extracted in a circular aperture of $\sim$ 1.2" ($\sim$ 2.2 kpc) in diameter, show signatures of high velocity winds in the form of broad (full width at half maximum; 1300$\leq$FWHM$\leq$2240 km/s and blueshifted components. We find that 4 out of the 5 QSO2s present outflows that we can resolve with our seeing-limited data, and they have radii ranging from 3.1 to 12.6 kpc. In the case of the two QSO2s with extended radio emission, we find that it is well-aligned with the outflows, suggesting that low-power jets might be compressing and accelerating the ionized gas in these radio-quiet QSO2s. In the four QSO2s with spatially resolved outflows, we measure ionized mass outflow rates of 3.3-6.5 Msun/yr when we use [S~II]-based densities, and of 0.7-1.6 Msun/yr when trans-auroral line-based densities are considered instead. We compare them with the corresponding molecular mass outflow rates (8 - 16 Msun/yr), derived from CO(2-1) ALMA observations at 0.2" resolution. Both phases show lower outflow mass rates than those expected from observational scaling relations where uniform assumptions on the outflow properties were adopted. This might be indicating that the AGN luminosity is not the only driver of massive outflows and/or that these relations need to be re-scaled using accurate outflow properties. We do not find a significant impact of the outflows on the global star formation rates.

==> trash/tab1old.tex <==
\begin{table}
  \caption{Main properties of the 3C sub sample observed with MUSE} 
  \begin{center}
\begin{tabular}{l c c c c c c c c}
\hline
Name  &  z   & Class & L$_{\rm bol}$ & Seeing  & scale\\
      &      &       &[erg s$^{-1}$]  & $\arcsec$ & kpc/1$\arcsec$ \\
\hline
3C~015    & 0.073  & LEG & 44.14 &   0.65 & 1.36\\ 
3C~017    & 0.220  & BLO & 45.53 &   0.49 & 3.37\\  
3C~018    & 0.188  & BLO & 46.09 &   0.53 & 3.00\\ 
3C~029    & 0.045  & LEG & 43.63 &   0.51 & 0.88\\ 
3C~033    & 0.060  & HEG & 45.72 &   0.63 & 1.14\\ 
3C~040    & 0.018  & LEG & 42.76 &   0.40 & 0.36\\ 
3C~063    & 0.175  & HEG & 45.17 &   0.49 & 1.36\\
3C~076.1  & 0.032  &  -- & 43.39 &   0.63 & 0.62\\
3C~078    & 0.029  & LEG & 42.95 &   0.53 & 0.57\\
3C~079    & 0.256  & HEG & 46.40 &   0.66 & 3.75\\
3C~088    & 0.030  & LEG & 43.68 &   0.59 & 0.60\\
3C~089    & 0.139  &  -- & 44.05 &   0.64 & 2.35\\
3C~098    & 0.030  & HEG & 44.54 &   0.66 & 0.60\\
3C~105    & 0.089  & HEG & 44.99 &   0.71 & 1.63\\
3C~135    & 0.127  & HEG & 45.59 &   0.52 & 2.20\\
3C~180    & 0.220  & HEG & 45.88 &   1.45 & 3.37\\
3C~196.1  & 0.198  & LEG & 45.06 &   0.48 & 3.12\\
3C~198    & 0.081  &  SF & 44.51 &   0.78 & 1.48\\
3C~227    & 0.086  & BLO & 45.29 &   0.91 & 1.58\\
3C~264    & 0.022  & LEG & 42.74 &   0.85 & 0.44\\
3C~272.1  & 0.003  & LEG & 41.74 &   0.39 & 0.07\\
3C~287.1  & 0.215  & BLO & 45.27 &   0.65 & 3.31\\
3C~296    & 0.025  & LEG & 43.32 &   1.08 & 0.49\\
3C~300    & 0.270  & HEG & 45.55 &   0.41 & 3.88\\
3C~318.1  & 0.045  &  -- & 42.90 &   1.38 & 0.86\\ 
3C~327    & 0.105  & HEG & 45.78 &   0.70 & 1.87\\  
3C~348    & 0.155  & LEG & 43.94 &   1.76 & 2.56\\  
3C~353    & 0.030  & LEG & 43.68 &   1.30 & 0.59\\ 
3C~386    & 0.017  &  -- & 43.74 &   0.61 & 0.34\\  
3C~403    & 0.059  & HEG & 45.29 &   0.54 & 1.13\\   
3C~403.1  & 0.055  & LEG & 43.40 &   0.80 & 1.04\\  
3C~424    & 0.127  & LEG & 44.35 &   0.98 & 1.20\\  
3C~442    & 0.026  & LEG & 42.75 &   0.61 & 0.51\\  
3C~445    & 0.056  & BLO & 46.04 &   1.48 & 1.07\\  
3C~456    & 0.233  & HEG & 46.35 &   1.27 & 3.51\\   
3C~458    & 0.289  & HEG & 45.57 &   0.50 & 4.07\\   
3C~459    & 0.220  & BLO & 45.57 &   0.43 & 3.37\\   
\hline
\end{tabular}
\end{center}
Column description: (1) source name; (2) redshift; (3) excitation
class (in some cases the strength of the emission lines is
insufficient to lead to a robust spectroscopic classification) from
\citet{Buttiglione10}; (4) bolometric luminosity obtained from nuclear
      [O~III] luminosity from \citet{Buttiglione10} multiplied by a
      factor 3500; (5) emission angle of the radio jets; (6) emssion
      angle of the outflowing gas; (7) date of the observation; (8)
      mean seeing of the observation; (9) conversion factor from
      $\ arcsec $ to kpc.
\label{tab:sample} 
\end{table}


==> trash/tab3old.tex <==
 \begin{table*}
  \caption{Properties of the extended outflows}
  \begin{center}
\begin{tabular}{l c c c r r r r r r}
\hline
Name    & Class & $M_{\text{of}}$  & $E_{\text{kin}}$& $R_{\rm out}$& $v_{\rm max}$ & Log $\dot{M}_{\rm of}$ & Log $\dot{E}_{\rm kin}$ & PA jet & PA outflow\\
        &       & [M$_{\odot}$] & [erg]  & [kpc]  & [km $s^{-1}$] & [M$_{\odot} s^{-1}$] & [erg s$^{-1}$] & [deg] & [deg] \\
\hline
%3C~015*    &   LEG  &	      & 	&$<$1.0  &  ~890~$\pm$~180  &	      &           & 152 &  -- \\ 
%3C~029*    &   LEG  &        &         &$<$0.2  &  ~880~$\pm$~170  &         &       & 160 &  -- \\ 
%3C~088*    &   LEG  &        &         &$<$0.7  &  1360~$\pm$~270  &         &       &  55 &  -- \\
%3C~196.1*  &   LEG  &        &         &$<$1.8  &  ~640~$\pm$~130  &         &       &  45 & --  \\
%\hline                                                                                        
%3C~017*    &   BLO  &        &         &$<$1.7  &  1100~$\pm$~220  &         &       & 156 &  -- \\  
%3C~018*    &   BLO  &        &         &$<$2.5  &  1120~$\pm$~220  &         &       & 163 &  -- \\
3C~227      &   BLO  & 5.55   &  53.78  &   2.5  &  1920~$\pm$~380  & -0.84   & 42.39 &  85 & --  \\   %diff
%3C~287.1*  &   BLO  &        &         &$<$2.4  &  1770~$\pm$~350  &         &       &  90 & --  \\
3C~445      &   BLO  & 5.79   &  52.61  &   4.3  &  2160~$\pm$~430  & -0.77   & 41.78 & 173 & 160?  \\ %?
3C~459      &   BLO  & 6.01   &  54.84  &   2.9  &  2040~$\pm$~410  & -0.26   & 42.68 &  97 & 110?  \\ %fil
\hline                                                                                        
3C~033      &   HEG  & 6.59   &  53.94  &   3.9  &  2000~$\pm$~400  & -0.17   & 42.38 &  19 &  61 \\   %bip
3C~063      &   HEG  & 5.78   &  54.74  &   1.1  &  1930~$\pm$~390  & -0.39   & 42.75 &  33 &  20? \\  %elong
3C~079      &   HEG  & 6.49   &  53.95  &   7.5  &  2450~$\pm$~490  & -0.34   & 42.4  & 105 &  47 \\   %fil
3C~098      &   HEG  & 4.38   &  52.28  &   0.6  &  2140~$\pm$~430  & -1.25   & 41.37 &  25 &     \\   %diff
3C~105      &   HEG  & 4.25   &  52.36  &   1.3  &  1910~$\pm$~380  & -2.1    & 40.35 & 127 &  -- \\   %diff
3C~135      &   HEG  & 5.40   &  52.65  &   2.2  &  1940~$\pm$~390  & -1.45   & 40.65 &  75 & 40  \\   %bip
3C~180      &   HEG  & 6.15   &  53.47  &   8.5  &  2450~$\pm$~490  & -1.28   & 41.13 &  10 & 29  \\   %bip
3C~300      &   HEG  & 6.25   &  54.88  &  14.0  &  2160~$\pm$~430  & -0.69   & 42.93 & 132 & 110?  \\ %fil/bip
3C~327      &   HEG  & 5.79   &  53.78  &   3.7  &  1440~$\pm$~290  & -0.8    & 41.95 & 100 & 62  \\   %bip
3C~403      &   HEG  & 5.03   &  53.37  &   1.1  &  1930~$\pm$~390  & -1.66   & 41.27 &  86 & 30?  \\  %fil 
%3C~456*    &   HEG  &  &  &$<$7.0  &  1900~$\pm$~380  &  &  &  17 & 135 \\   
\hline
 \label{table:estese}
\end{tabular}
\end{center}
Column description: (1) source name; (2) excitation class; (3) mass of
outflowing ionized gas; (4) kinetic energy of the outflow; (5)
extension of the outflow from the nucleus; (6) maximum value of the
median velocity ($v_{50}$) reached by the outflow; (7 and 8) mass and
energy rate of the outflow; (9 and 10) position angle of the radio
axis and of the extended outflow. The * indicates that sources very
compact whose outflow extension is considered as an upper limit.
\label{tab:estese} 
\end{table*}






==> trash/tab4old.tex <==
 \begin{table*}
  \caption{Energetical properties of the outflows}
  \begin{center}
\begin{tabular}{l c c c r r r r r }
\hline
Name    & Class & Log $M_{\text{of}}$   & Log $E_{\text{kin}}$ & R$_{out}$ & Log $\dot{E}_{\rm kin}$ &  $\dot{M}_{\rm of}$ &  Log $\dot{P}_{\rm of}$ &  Log $\dot{P}_{\rm AGN}$  \\
        &       &  [M$_{\odot}$]   &  [erg]          & [kpc]    & [erg s$^{-1}$]          &   [M$_{\odot} yr^{-1}$] &  [dyn]]                &  (L$_{bol}$/c)            \\
\hline
3C~015   & LEG  & 5.7    & 54.3     &$<$3.8  & $>$40.6 &  $>$0.4  & $>$33.1  &  34.6 \\
3C~017   & BLO  & 6.7    & 55.2     &$<$18.5 & $>$41.2 &  $>$1.6  & $>$33.8  &  36.0 \\
3C~018   & BLO  & 6.5    & 55.3     &$<$15.7 & $>$41.4 &  $>$1.5  & $>$33.9  &  36.2 \\
3C~029   & LEG  & 4.9    & 53.4     &$<$1.2  & $>$40.1 &  $>$0.1  & $>$32.6  &  33.7 \\
3C~033   & HEG  & 8.2    & 56.0     &3.8     & 44.5    &  30.8    & 34.6     &  35.5 \\
3C~040   & LEG  & $<$3.5 & $<$52.6  &$<$0.2  &  --     &  --      & --       &  32.8 \\
3C~063   & HEG  & 7.3    & 56.3     &4.3     & 44.3    &  14.6    & 35.0     &  35.5 \\
3C~076.1 & OTH  & $<$4.6 & $<$52.7  &$<$0.8  &  --     &  --      & --       &  33.2 \\
3C~078   & LEG  & $<$4.3 & $<$53.0  &$<$0.5  &  --     &  --      & --       &  33.8 \\
3C~079   & HEG  & 8.1    & 55.8     &4.6     & 44.5    &  19.2    & 34.4     &  36.8 \\
3C~088   & LEG  & 4.4    & 53.1     &$<$0.6  & $>$39.9 &  $>$0.1  & $>$32.4  &  33.9 \\
3C~89    & OTH  & $<$6.2 & $<$55.1  &$<$11.4 &  --     &  --      & --       &  33.4 \\
3C~098   & HEG  & 5.7    & 53.6     &0.4     & 42.7    &  1.1     & 33.3     &  34.7 \\
3C~105   & HEG  & 6.0    & 54.1     &2.1     & 42.2    &  0.5     & 33.0     &  34.9 \\
3C~135   & HEG  & 7.2    & 54.9     &4.8     & 42.9    &  2.4     & 33.5     &  35.7 \\
3C~180   & HEG  & 7.9    & 55.6     &16.3    & 43.6    &  3.2     & 33.6     &  36.7 \\
3C~196.1 & LEG  & 5.9    & 54.0     &$<$15.4 & $>$39.9 &  $>$0.2  & $>$32.6  &  35.4 \\
3C~198   & SF   & $<$5.7 & $<$53.5  &$<$5.5  &  --     &  --      & --       &  35.1 \\
3C~227   & BLO  & 7.2    & 55.5     &2.8     & 44.1    &  7.1     & 34.2     &  36.0 \\
3C~264   & LEG  & $<$4.1 & $<$52.3  &$<$0.5  &  --     &  --      & --       &  32.9 \\
3C~272   & LEG  & $<$2.4 & $<$50.0  &$<$0.0  &  --     &  --      & --       &  30.8 \\
3C~2871  & BLO  & $<$5.6 & $<$53.8  &$<$23.9 &  --     &  --      & --       &  35.0 \\
3C~296   & LEG  & $<$4.2 & $<$52.3  &$<$0.8  &  --     &  --      & --       &  33.8 \\
3C~300   & HEG  & 7.9    & 56.7     &20.2    & 45.0    &  8.2     & 34.6     &  35.9 \\
3C~327   & HEG  & 7.6    & 55.5     &3.5     & 43.9    &  9.6     & 34.2     &  36.1 \\
3C~348   & LEG  & $<$6.2 & $<$55.2  &$<$38.1 &  --     &  --      & --       &  34.4 \\
3C~353   & LEG  & $<$4.4 & $<$53.2  &$<$1.4  &  --     &  --      & --       &  33.8 \\
3C~403   & HEG  & 6.7    & 55.1     &1.3     & 43.0    &  1.2     & 33.4     &  35.3 \\
3C~403.1 & LEG  & $<$5.1 & $<$54.2  &$<$2.7  &  --     &  --      & --       &  32.5 \\
3C~424   & LEG  & $<$4.4 & $<$52.2  &$<$15.2 &  --     &  --      & --       &  33.9 \\
3C~442   & LEG  & 4.5    & 52.7     &$<$0.5  & $>$39.3 &  $>$0.0  & $>$32.0  &  33.3 \\
3C~445   & BLO  & 7.5    & 55.1     &1.5     & 44.2    &  9.2     & 33.9     &  36.5 \\
3C~456   & HEG  & 6.2    & 55.0     &$<$52.5 & $>$40.8 &  $>$0.3  & $>$33.2  &  37.2 \\
3C~458   & HEG  & $<$5.9 & $<$54.0  &$<$28.3 &  --     &  --      & --       &  35.6 \\
3C~459   & BLO  & 7.7    & 56.4     &3.0     & 44.4    & 25.7     & 34.9     &  35.7 \\
\hline
 \label{table:estese}
\end{tabular}
\end{center}
Column description: (1) source name; (2) excitation class; (3) mass of
outflowing ionized gas; (4) kinetic energy of the outflow; (5)
extension of the outflow from the nucleus; (6) maximum value of the
median velocity ($v_{50}$) reached by the outflow; (7 and 8) mass and
energy rate of the outflow; (9 and 10) position angle of the radio
axis and of the extended outflow. The * indicates that sources very
compact whose outflow extension is considered as an upper limit.
\label{tab:estese} 
\end{table*}







































